Visual Storytelling via Predicting Anchor Word Embeddings in the Stories

We propose a learning model for the task of visual storytelling. The main idea is to predict anchor word embeddings from the images and use the embeddings and the image features jointly to generate narrative sentences. We use the embeddings of randomly sampled nouns from the groundtruth stories as the target anchor word embeddings to learn the predictor. To narrate a sequence of images, we use the predicted anchor word embeddings and the image features as the joint input to a seq2seq model. As opposed to state-of-the-art methods, the proposed model is simple in design, easy to optimize, and attains the best results in most automatic evaluation metrics. In human evaluation, the method also outperforms competing methods.

==> vis.tex <==
% !TEX root = main.tex

\begin{figure*}
	\centering
	\begin{tabular}{p{\textwidth}}
		\toprule
		\raisebox{-.5\height}{\includegraphics[width=1\textwidth]{files/vis/vis_1.pdf}} \\
		\small
    \textbf{Story by human:}  The bazzar was filled with many unique items. Because of the rain, few people came out. As the rain cleared it began to get crowded. [male] found a unique stall. The owner was a crochety old lady. \\[2pt]
		\small
    \textbf{AREL\cite{wang2018no}:} {\color{blue}There were a lot of people} at the market today. {\color{blue} We had a lot of people there. There were a lot of people there.} The food was delicious. We had a lot of fun. \\[2pt]
		\small
    \textbf{StoryAnchor: Image Only:}  We went to the local market today. {\color{blue} There were a lot of people there. There was a lot of people there.} We had a lot of food to choose from. I had a great time there. \\[2pt]
		\small
    \textbf{StoryAnchor: w/ Predicted Nouns:} We went to the market to get some groceries. {\color{blue} There was a lot of people} at the market. The streets were filled with people. {\color{blue} There were a lot of people there.} The kids were very excited to see them. \\[2pt]
		\small
    \textbf{StoryAnchor: w/ Ground-truth Nouns:} We went to the local market to buy some food items. {\color{blue} The rain was rain, but the rain was rain. The rain started to rain.} [male]'s favorite part of the day was the local restaurant. The owner of the owner was very happy to see him. \\[2pt]
    \midrule
		\small
    \textbf{Predicted Nouns:} something; something; something; what; what\\[2pt]
		\small
    \textbf{Ground-truth Nouns:} items; rain; rain; [male]; owner\\
	\bottomrule
	\end{tabular}
	\begin{tabular}{p{\textwidth}}
		\toprule
		\small
		\raisebox{-.5\height}{\includegraphics[width=1\textwidth]{files/vis/vis_2.pdf}} \\
    \small \textbf{Story human:}  This year she brought her dog to watch the halloween dog parade. There are so many cute costumes, like this little devil. This dog looks just like a jack 'o lantern. Some dogs prefer a more `royal' look. But the winner of this years award for cute, goes to this little prisoner.\\[2pt]
    \small \textbf{AREL\cite{wang2018no}:} I went to the park yesterday. {\color{blue}Even the dog was excited to see him. Even the dog was excited to see him.} The dogs were so happy to be there. And the dog had a good time. \\[2pt]
    \small \textbf{StoryAnchor: Image Only:} This is a picture of a man. He even got to pet the dog. I took a picture of the dog. He even brought a dog with his dog. The dog had a great time. \\[2pt]
    \small \textbf{StoryAnchor: w/ Predicted Nouns:} This was my first day of the year. {\color{blue} The dog was so excited to be there. Even the dog was excited to be there.} This is [male]'s dog. The dog had a great time.\\[2pt]
    \small \textbf{StoryAnchor: w/ Ground-truth Nouns:} This year, I went to a halloween party this year. The dog was cute and cute. {\color{blue}Even the dog was very happy. Even the dogs were very happy.} Even the dog had a good time. \\[2pt]
    \midrule
    \small \textbf{Predicted Nouns:} momentous; extended; something; something; something;\\[2pt]
    \small \textbf{Ground-truth Nouns:} year; cute; dog; dogs; UNK\\
		\bottomrule
	\end{tabular}

	\caption{Qualitative visualization of narrative stories generated by human and different methods. Similar sentences for similar images are annoated in {\color{blue} blue}.}
	\label{fig:vis_1}
\end{figure*}


\begin{figure*}
	\centering
	\begin{tabular}{p{\textwidth}}
		\toprule
		\raisebox{-.5\height}{\includegraphics[width=1\textwidth]{files/vis/vis_3.pdf}} \\
		\small
    \textbf{Story human:} It was the day my boy graduated. I kept the pamphlet that had his name in it. The faculty congratulated my boy on his work. He looked so proud on that stage. I hope that his smile lasts long into his adulthood.\\[2pt]
		\small
    \textbf{AREL\cite{wang2018no}:} The awards ceremony was held at the organization. They were a lot of people there. We had a lot of people there. The president of the school was a lot of fun. I had a great time. \\[2pt]
		\small
    \textbf{StoryAnchor: Image Only:} I had a great time at the graduation ceremony. The plaque was the. He was very happy to be there. He was very proud of his accomplishments. I had a great time there.\\[2pt]
		\small
    \textbf{StoryAnchor: w/ Predicted Nouns:} Today was the day of the graduation. It was a very special day. We were so happy to be there. The man and his wife were there to celebrate their accomplishments. Everyone was very happy to be there.\\[2pt]
		\small
    \textbf{StoryAnchor: w/ Ground-truth Nouns:} Today was the day of the graduation. {\color{red} We had a pamphlet at the reception. The boy was so happy to be there. He was so excited to see the stage}. I was so happy to be there. \\[2pt]
    \midrule
		\small
    \textbf{Predicted Nouns:}  I; UNK; momentous; momentous; wally \\[2pt]
		\small
    \textbf{Ground-truth Nouns:} boy; pamphlet; boy; stage; smile\\[2pt]
		\bottomrule
	\end{tabular}

	\caption{Qualitative visualization of good quality stories that are generated with anchor words. The sentences with anchor words are annotated as {\color{red}red} in the generated stories.}
	\label{fig:vis_2}
\end{figure*}

